When Compression Helps and When It Hurts: Condition-Aware Analysis of Chain-of-Thought Distillation

Chain-of-Thought (CoT) distillation transfers multi-step reasoning from large reasoning models to smaller students, but verbose teacher traces inflate both training and inference cost. Existing CoT compression methods fall into two families, selective pruning and generative rewriting, yet prior studies have left key factors entangled: granularity is confounded with importance criteria in pruning, restructuring level is rarely isolated in rewriting, and compression budgets are not systematically evaluated across domains or regimes. We recast CoT compression along three dimensions: importance criterion, restructuring level, and compression budget. Sweeping these across two model families, Math and General domains, and Long-/Short-CoT regimes, we find that (i) importance criterion utility is strictly governed by granularity: step-level criteria converge on a shared reasoning backbone, while token-level pruning requires symbol-aware signals to preserve the logical core; (ii) restructuring level inverts across domains: Math degrades monotonically with structural disruption, while aggressive rewriting acts as a denoiser on General tasks; (iii) training-time compression does not necessarily translate to inference-time savings: Long-CoT students retain verbose habits despite concise supervision, making the training ratio an optimistic lower bound on deployment cost. These findings yield condition-aware guidelines for matching compression to deployment context.

==> Sections/Act-III.tex <==
\section{Act III: CoT-level Factor Analysis}
\label{sec:Act-III}

\subsection{Measurement setup: CoT sampling and factor definitions}

\subsection{Structural preservation as the primary driver (Math vs. General)}

\subsection{Coherence and redundancy: why General tolerates aggressive rewriting}
% R1-compress more like language-model coherence / token-level consistency, i.e., how well a compressed CoT supports reconstructing the original teacher CoT under a strong LM.

% But mine is like reasoning coherence as supervision: how clear and easy-to-follow a compressed CoT is as a standalone reasoning trace for a smaller model.

% So we care more about how students can learn a stable reasoning regime from those pruned cots. Therefore, we use LLM-judge as the indicator of how well the coherence in cot is.

% We do a compare in the appendix between the LLM judge and loss coherence compare.
% % 对 General 任务，算一下 LM-based token loss（类似 R1 的做法）+ LLM-judge coherence，看这俩和 accuracy 的相关性；
% % 告诉读者：LM loss 和 judge coherence 在 General 上相关性还可以，在 Math 上明显变弱；
% % 进一步 justify：为什么我们主文选择 LLM judge 作为 coherence 因子。

\subsubsection{Measurement: LLM-judged coherence.}
Prior work such as R1-Compress~\citep{wang2025r1compresslongchainofthoughtcompression} measures the ``coherence'' of compressed CoTs via token-level language-model loss: given a compressed trace as context and the original CoT as reference, a strong LM is used to evaluate the average log-likelihood of the original tokens. Lower loss is interpreted as higher token-level coherence and better inter-chunk consistency.

In our setting, however, we are primarily interested in \emph{reasoning coherence as supervision}: how clear and easy to follow a compressed CoT for a smaller student model, irrespective of how closely it matches the teacher's surface form. We therefore rely on an
LLM judge to provide pairwise coherence comparisons between CoTs and derive a coherence win-rate for each method. 

We therefore evaluate the readability of compressed CoTs using an LLM-as-a-judge protocol.
For each input $x$, we compare a method's CoT $y_{\text{meth}}$ against a reference
trace $y_{\text{ref}}$ (either the teacher CoT or a strong structure-preserving
baseline). A high-capacity LLM is asked to decide which of the two traces is more
logically coherent as a step-by-step explanation (full prompt provided in
Appendix~\S\ref{app:judge-prompt}).

The judge outputs one of \texttt{A\_better}, \texttt{B\_better}, or \texttt{tie}.
For each pruning method, we report a \emph{coherence win-rate}: the fraction of
comparisons in which $y_{\text{meth}}$ is preferred over the reference (ties counted
as non-wins). This yields an ordinal, pairwise-comparable measure of coherence within
each domain and method family, without assigning absolute quality labels.

\vspace{0.5em}
\paragraph{Finding 1: Globally, coherence is only a weak proxy for accuracy.}
Across methods and domains, judged coherence shows only weak alignment with downstream accuracy.
Highly compressed token-level extraction traces often have near-zero coherence win-rate but can
match the accuracy of more coherent summarization baselines at similar token budgets on some
benchmarks; conversely, some high-coherence rewrites can hurt accuracy, especially on Math tasks. Thus, coherence is not a universal performance surrogate—it must be interpreted in the context of the pruning paradigm and domain.

\vspace{0.5em}
\paragraph{Finding 2: For extraction, Math behaves as coherence-sensitive, General as coherence-robust.}
Within the extraction family, coherence behaves like a \emph{damage indicator}, and this effect is strongly domain-dependent.
For extraction on Math, however, coherence behaves like a damage indicator:
once judged coherence drops to very low levels (as in token-level LLMLingua2), accuracy almost always collapses.
In contrast, General-domain benchmarks are more robust: even highly compressed, low-coherence token extraction can still match the accuracy of more coherent methods at similar token budgets.

\vspace{0.5em}
\paragraph{Finding 3: For summarization, coherence is necessary but far from sufficient.}
In contrast, within the summarization family judged coherence plays more of a gatekeeping role.

Methods like structure-none rewriting can achieve reasonable coherence scores while still hurting Math accuracy, suggesting that structural fidelity and domain-specific reasoning requirements dominate once a basic level of coherence is satisfied.

\vspace{0.5em}
\paragraph{Takeaway.}
Judged coherence is best viewed as a second-order explanatory factor that interacts with both the
pruning paradigm and the domain.
For extraction on Math, it reliably signals harmful compression, whereas General-domain tasks are
much more tolerant to low-coherence scripts. 
For summarization, coherence mainly ensures that rewrites remain readable, while structural
preservation and task-specific reasoning demands ultimately determine whether compressed CoTs
translate into accurate, token-efficient student models.


\subsection{Reflection and verification steps: linking long-CoT training to compressibility}

\subsection{Combined view and design rules}

==> Sections/Experiments.tex <==
\section{Experimental Setup}

\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{fig/figure_subplot_improve_drop.pdf}
\caption{Comparison of summarization- and extraction-based CoT compression across domains and training regimes. Each subplot reports accuracy under different prune ratios on Math/General $\times$ Short/Long settings. Bars show accuracy at prune ratios $0.5/0.7/0.9$, and the orange line shows the corresponding inference token ratio.}
\vspace{-12pt}
\label{fig:2*2_drop}
\end{figure*}

\subsection{Models, Data, and Metrics}
\paragraph{Student Models.}
We employ LLaMA-3.1-8B-Instruct~\citep{dubey:2024llama3} as the primary student model, with the Qwen2.5 series~\citep{Qwen2.5} used to verify cross-model and scale generalization; full results are provided in Appendix~\ref{appendix:Result_equation}).

\paragraph{Training Corpora.} 
To analyze the impact of reasoning length, we construct two training sets: a Short-CoT regime sampled from Natural Reasoning~\citep{yuan2025naturalreasoningreasoningwild28m} (5k instances), and a Long-CoT regime from LIMO~\citep{ye2025limoreasoning}.

\paragraph{Evaluation Benchmarks}
The evaluation spans five benchmarks in two domains:
(1) Math: GSM8K, MATH500 for \textit{short-CoT} regime and MATH500, AMC23, AIME24 for \textit{long-CoT} regime;(2) General: GPQA Diamond and MMLU-PRO for both regimes.

\paragraph{Evaluation Metrics.}
We report Accuracy for reasoning quality and the Inference Token Ratio ($\rho_{\text{inference}}$)—the ratio of generated tokens relative to the uncompressed baseline—for cost efficiency.

\subsection{\texorpdfstring{Compression Strategies ($\phi$)}{Compression Strategies (phi)}}
We implement two compression paradigms defined in Section~\ref{sec:formulation}:
\begin{itemize}[leftmargin=*, nosep]
\item \textbf{Extraction ($\phi_{\text{importance}}$):} We prune tokens or steps based on three importance scores: LLMLingua2 (learned saliency), Entropy (uncertainty) and NLL (surprise).
% \item \textbf{Summarization ($\phi_{\text{structure}}$):} We utilize Gemini 2.5 Flash to rewrite traces into four structural fidelity levels: Structural Preservation (SP), Editing (SE), Semantic Fusion (SF), and Framework Replacement (FR).
\item \textbf{Summarization ($\phi_{\text{restruct}}$):} We utilize Gemini 2.5 Flash ~\citep{comanici2025gemini25pushingfrontier} as the primary rewriter to rewrite traces into four restructuring levels: Structural Preservation, Structural Editing, Semantic Fusion, and Framework Replacement. We additionally verify using GPT-4o-mini~(\citealt{openai2024gpt4o}) in Appendix~\ref{appendix:cross_rewriter}.
\end{itemize}

\subsection{Implementation Details}We fine-tune all models via LoRA~\citep{lora}. Evaluation uses a standardized greedy-like decoding with temperature 0.7. Full hyperparameters, prompt templates for rewriting, and redundancy signals definitions are provided in Appendix~\ref{appendix:training_details}.









==> inputs/recovery-gpt.tex <==
\begin{figure}[htbp]
\begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black,title=Revovering the Compressed Chain-of-Thought,fontupper=\footnotesize,fonttitle=\scriptsize]
\textbf{Compressed CoT}: break down Deanna 26 Marcus five younger 26 - 5 21 Marcus half Leo's age twice Marcus Marcus 21, Leo's age 2 x 21 = 42.

\vskip 0.1in
        
\textbf{Recovered CoT}: 1. We know that Deanna is 26 years old. 2. Marcus is five years younger than Deanna. So, Marcus’s age is \( 26 - 5 = 21 \). 3. Marcus is also half of Leo’s age, which means Leo’s age is twice Marcus’s age. 4. Since Marcus is 21 years old, Leo’s age is \( 2 \times 21 = 42 \). So, Leo is 42 years old.
\end{tcolorbox}
\vskip -0.1in
\caption{Recovering the compressed CoT for GSM8K math word problem using GPT-4o.}
\vskip -0.1in
\label{fig:recovery-gpt}
\end{figure}

==> inputs/recovery-prompt.tex <==
\begin{figure}[htbp]
\begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black,title=Input Prompt for CoT Recovery,fontupper=\footnotesize,fonttitle=\scriptsize]
Could you please recover the following compressed Chain-of-Thought output of a mathematical question to its original full content?

\vskip 0.1in

The question is: 

Marcus is half of Leo’s age and five years younger than Deanna. Deanna is 26. How old is Leo?

\vskip 0.1in

The compressed Chain-of-Thought: 

break down Deanna 26 Marcus five years younger 26 - 5 21 Marcus half Leo's age Leo twice Marcus's age Marcus 21, Leo's age 2 x 21 = 42.

\vskip 0.1in

Original Full Chain-of-Thought:
\end{tcolorbox}
\vskip -0.1in
\caption{Input prompt for LLaMA-3.1-8B-Instruct designed to recover the compressed CoT from a GSM8K math problem.}
\vskip -0.1in
\label{fig:recovery-prompt}
\end{figure}

==> inputs/recovery.tex <==
\begin{figure}[t]
\begin{tcolorbox}[colback=blue!5!white,colframe=blue!75!black,title=Revovering the Compressed Chain-of-Thought,fontupper=\footnotesize,fonttitle=\scriptsize]
\textbf{Compressed CoT}: break down Deanna 26 Marcus five younger 26 - 5 21 Marcus half Leo's age twice Marcus Marcus 21, Leo's age 2 x 21 = 42.

\vskip 0.1in
        
\textbf{Recovered Compressed CoT}: Let's break it down step by step. Deanna is 26 years old. Marcus is five years younger than Deanna: M = D - 5. Marcus's age: M = 26 - 5 = 21. Marcus is half of Leo's age: M = L / 2. Leo is twice Marcus's age: L = 2M. Leo's age: L = 2 x 21 = 42.

\end{tcolorbox}
\caption{Recovering the compressed CoT for GSM8K math word problem using LLaMA-3.1-8B-Instruct.}
\label{fig:recovery}
\end{figure}

==> inputs/text_file/token_importance_llama.tex <==
\colorize{100}{Let}
\colorize{10.6}{'s}
\colorize{58.2}{break}
\colorize{20.8}{it}
\colorize{2}{down}
\colorize{37.9}{step}
\colorize{16}{by}
\colorize{0}{step}
\colorize{41.4}{:}
\colorize{4.6}{1.}
\colorize{100}{Deanna}
\colorize{36.8}{is}
\colorize{48.8}{26}
\colorize{8.6}{years}
\colorize{0}{old}
\colorize{14.6}{.}
\colorize{100}{2.}
\colorize{100}{Marcus}
\colorize{48.0}{is}
\colorize{92.8}{five}
\colorize{3.15}{years}
\colorize{28.7}{younger}
\colorize{0}{than}
\colorize{91.9}{Deanna}
\colorize{15.4}{,}
\colorize{38.9}{so}
\colorize{29.9}{Marcus}
\colorize{4.30}{is}
\colorize{65.5}{26}
\colorize{22.9}{-}
\colorize{1.32}{5}
\colorize{0}{=}
\colorize{0}{21}
\colorize{2.4}{years}
\colorize{2.5}{old}
\colorize{9.3}{.}
\colorize{100}{3.}
\colorize{87.8}{Marcus}
\colorize{41.9}{is}
\colorize{87.1}{half}
\colorize{9.8}{of}
\colorize{100}{Leo}
\colorize{31.8}{'s}
\colorize{0.1}{age}
\colorize{15.1}{,}
\colorize{30.1}{so}
\colorize{12.4}{Leo}
\colorize{14.8}{'s}
\colorize{0}{age}
\colorize{3}{is}
\colorize{12.0}{twice}
\colorize{4.8}{Marcus}
\colorize{3.8}{'s}
\colorize{1.2}{age}
\colorize{3.2}{.}
\colorize{100}{4.}
\colorize{76.6}{Since}
\colorize{100}{Marcus}
\colorize{27.8}{is}
\colorize{38.4}{21,}
\colorize{74.2}{Leo}
\colorize{23.6}{'s}
\colorize{3.1}{age}
\colorize{8.0}{is}
\colorize{22.0}{2}
\colorize{39.0}{x}
\colorize{6.7}{21}
\colorize{6.0}{=}
\colorize{0}{42}
\colorize{9.0}{.}
(Selective Context)


==> inputs/text_file/token_importance_llmlingua.tex <==
\colorize{0.7}{Let}
\colorize{2.4}{'s}
\colorize{98.9}{break}
\colorize{11.0}{it}
\colorize{90.3}{down}
\colorize{50.4}{step}
\colorize{39.7}{by}
\colorize{31.9}{step}
\colorize{20.7}{:}
\colorize{47.8}{1.}
\colorize{100}{Deanna}
\colorize{1.6}{is}
\colorize{100}{26}
\colorize{71.0}{years}
\colorize{83.5}{old}
\colorize{25.3}{.}
\colorize{24.7}{2.}
\colorize{100}{Marcus}
\colorize{7.8}{is}
\colorize{96.7}{five}
\colorize{86.6}{years}
\colorize{98.8}{younger}
\colorize{4.4}{than}
\colorize{42.2}{Deanna}
\colorize{6.4}{,}
\colorize{1.3}{so}
\colorize{57.5}{Marcus}
\colorize{1.9}{is}
\colorize{98.2}{26}
\colorize{98.1}{-}
\colorize{97.0}{5}
\colorize{84.9}{=}
\colorize{99.8}{21}
\colorize{74.0}{years}
\colorize{77.5}{old}
\colorize{27.3}{.}
\colorize{21.2}{3.}
\colorize{96.4}{Marcus}
\colorize{7.9}{is}
\colorize{98.0}{half}
\colorize{19.1}{of}
\colorize{99.6}{Leo}
\colorize{94.6}{'s}
\colorize{97.9}{age}
\colorize{3.2}{,}
\colorize{5.6}{so}
\colorize{88.2}{Leo}
\colorize{78.7}{'s}
\colorize{81.2}{age}
\colorize{1.5}{is}
\colorize{98.3}{twice}
\colorize{98.4}{Marcus}
\colorize{87.9}{'s}
\colorize{88.1}{age}
\colorize{73.3}{.}
\colorize{31.4}{4.}
\colorize{2.8}{Since}
\colorize{98.1}{Marcus}
\colorize{4.0}{is}
\colorize{98.2}{21,}
\colorize{98.5}{Leo}
\colorize{91.1}{'s}
\colorize{95.1}{age}
\colorize{3.4}{is}
\colorize{98.8}{2}
\colorize{98.5}{x}
\colorize{99.0}{21}
\colorize{94.6}{=}
\colorize{99.8}{42}
\colorize{98.3}{.}
(LLMLingua-2)


==> inputs/token-importance.tex <==
\begin{figure}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \fbox{\parbox[c]{1.1\columnwidth}{
        \textbf{Problem: } Marcus is half of Leo’s age and five years younger than Deanna. Deanna is 26. How old is Leo?

        \vskip 0.1in

        \textbf{Chain-of-Thought: } {\setlength{\fboxsep}{-1pt}
         \input{inputs/text_file/token_importance_llama}
        }

        \vskip 0.1in

        \textbf{Chain-of-Thought: } {\setlength{\fboxsep}{-1pt}
         \input{inputs/text_file/token_importance_llmlingua}
        }

        \vskip 0.05in

        \textbf{Final Answer: } 42.
    }}}
    \caption{Visualization of token importance within a CoT sequence, with darker colors indicating higher values. This figure compares two token importance measurements: Selective Context and LLMLingua-2.}
    \label{fig:token-importance}
\end{figure}
